DSP Implementation of a Direct Adaptive Feedfoward Control Algorithm for Rejecting Repeatable Runout in Hard Disk Drives

A direct adaptive feedforward control method for tracking repeatable runout (RRO) in bit patterned media recording (BPMR) hard disk drives (HDD) is proposed. The technique estimates the system parameters and the residual RRO simultaneously and constructs a feedforward signal based on a known regressor. An improved version of the proposed algorithm to avoid matrix inversion and reduce computation complexity is given. Results for both MATLAB simulation and digital signal processor (DSP) implementation are provided to verify the effectiveness of the proposed algorithm.

==> 4-Conclusion.tex <==
%=========================================================
\section{Conclusion}\label{sec:conclusion}
%=========================================================
